Voter Priming Campaigns: Strategies, Equilibria, and Algorithms

Issue salience is a major determinant in voters' decisions. Candidates and political parties campaign to shift salience to their advantage - a process termed priming. We study the dynamics, strategies and equilibria of campaign spending for voter priming in multi-issue multi-party settings. We consider both parliamentary elections, where parties aim to maximize their share of votes, and various settings for presidential elections, where the winner takes all. For parliamentary elections, we show that pure equilibrium spending always exists and can be computed in time linear in the number of voters. For two parties and all settings, a spending equilibrium exists such that each party invests only in a single issue, and an equilibrium can be computed in time that is polynomial in the number of issues and linear in the number of voters. We also show that in most presidential settings no equilibrium exists. Additional properties of optimal campaign strategies are also studied.

==> 2_candidates.tex <==
\section{Two Candidates}

\todo{Think again about how exactly we want to organize it. Perhaps some general lemmas and then within each section?}

In the case of only two candidates, the different utility functions results in an almost identical game.

\begin{definition}
    The \emph{weight} of an issue $i$ is $Q^*_i = \sum_{c \in C} Q_i^c$. Issue $i$ is \emph{heavier} than issue $j$ if $Q^*_i>Q^*_j$.
\end{definition}
\newcommand{\investin}[4]{\bm{w}(#1\shortto #2,#3\shortto #4)}
For candidates $c,c'$ and issues $i,i'$ denote $\investin{c}{i}{c'}{i'}$ the investment wherein $c$ investment all and only in $i$ and $c'$ all and only in $i'$.

\begin{lemma}
\label{lemma:investing_in_heavier_issue}
     For candidates $c,c'$ and issues $i, i', j, j'$, with $Q^*_i < Q^*_{i'}, Q^*_j < Q^*_{j'}$, if
     \begin{align}
     \upar^c(\investin{c}{i}{c'}{j})&<
     \upar^c(\investin{c}{i'}{c'}{j}) & \text{and},\\
     \upar^{c'}(\investin{c}{i'}{c'}{j})&<
     \upar^{c'}(\investin{c}{i'}{c'}{j'}) &
     \end{align}
Then
\begin{align}
     \upar^c(\investin{c}{i}{c'}{j'})&<
     \upar^c(\investin{c}{i'}{c'}{j'}) &
\end{align}
\end{lemma}

\begin{proof}
    Since candidates are investing in different issues ($c$ only in $i, i'$ and $c'$ only in $j, j'$), we can assume a budget of $1$ for every candidate, by %dividing every $Q^{c''}_{i''}$ by $W^c$ and $Q^{c''}_{j''}$ by $W^{c'}$, for every $c'' \in \{c, c'\}, i'' \in \{i, i'\}, j'' \in \{j, j'\}$.
    normalizing every issue accordingly (i.e. dividing the ranking of each player by the original budget).

    
\end{proof}

This lemma will allow us to compute the Nash equilibrium, as we later show.

\begin{theorem}
    \label{theroem:2-candidates-pure-strategies}
    In the case of two candidates there always exists a Nash equilibrium with pure strategies and focused investments.
\end{theorem}


\begin{theorem}
    \label{theorem}
    With two candidates a (pure-strategies and focused-investments) Nash equilibrium can be computed in time $O(|V||I|^2)$. 
\end{theorem}

\begin{algorithm}[ht]
\caption{\small{FindEquilibrium$(\cdot)$: Returns a pure Nash equilibrium with pure investments}\label{alg:mxrelaxpro}}
\begin{algorithmic}[1]
\REQUIRE Set of candidates: $C = \{c^1, c^2, ...\}$, vector of biases: $b$, array of issues $I = \{1, 2, ...\}$, advertisement budget of $c^1, c^2$: $a_1, a_2$.
\ENSURE A pair of issues $(i_1, i_2)$ such that investment of $c^1, c^2$ in $i_1, i_2$ correspondingly is a Nash equilibrium.

\STATE $c_0 \leftarrow 0 \hspace{1cm} \forall c \in C$
\STATE $I \leftarrow I \cup \{0\}$
\STATE $I \leftarrow Sort(I, key=\sum_{c \in C} c_i)$ 
\STATE $b_* \leftarrow \sum_{c \in C} B^c$
\STATE $c^*_i \leftarrow \sum_{c \in C} c_i \hspace{1cm} \forall i \in I$
\STATE $u(m, m', i, j) := \frac{a_m c^m_i + a_{m'} c^m_j}{a_m c^*i + a_{m'} c^*_j + b_*}$
\STATE $k_1 \leftarrow 0$
\STATE $k_2 \leftarrow 0$
\STATE $\text{continue} \leftarrow \TRUE$
\WHILE {$\text{continue}$}
    \STATE $\text{continue} \leftarrow \FALSE$
    \FOR {$m \in \{1, 2\}$}
        \STATE $m' \leftarrow (2, 1)_m$
        \STATE $k \leftarrow \argmax_{k \in I[k_m:]} u(m, m', I[k], I[k_{m'}])$
        \IF {$k_m \ne k$}
            \STATE $k_m \leftarrow k$
            \STATE $\text{continue} \leftarrow \TRUE$
        \ENDIF
    \ENDFOR
\ENDWHILE
\RETURN $(I[k_1], I[k_2])$\;
\end{algorithmic}
\end{algorithm}

==> proofs/frac/2_candidates_algorithm_complexity.tex <==
% \begin{proof}
%     By \cref{model:first_simplification} and \cref{model:final_simplification}, computing the simplified version of the problem takes $O(|V|)$ steps.

%     The first line of the algorithm takes $O(|I|)$ steps. For the second line, since in every iteration of the loop we advance either $i$ or $j$ and we do not repeat issues, the number of iterations is at most $2 \cdot |I|$. 
    
%     Computing the utility of candidates given focus investments is constant (as there are only two candidates), and is done for every issue, hence the first two steps in the loop takes $O(|I|)$ time each. Performing argmax over issues also take $O(|I|)$ time, hence every iteration takes $O(I)$ time, results in total time of $O(|I|^2)$ for the loop.
% \end{proof}

==> proofs/frac/focus_optimal_then_split_is_old.tex <==
The proof of the theorem rests on a series of lemmas and observations. The following is easy to show, based on the fact that constraints for feasible investments are linear.
\begin{observation}
    The feasible investments of a candidate $c$ form a convex space.
\end{observation}

\begin{lemma}
    \label{frac:best_middle_response}

    Given two feasible investments $\bm{x}, \bm{y}$ of $\bm{c}$, and an investment $\bm{z} = r \cdot \bm{x} + (1 - r) \cdot \bm{y} : 0 < r < 1$ between them, as responses against pure strategies $\bm{w^-c}$ of the other candidates, $\bm{z}$ is a best response if and only if $\bm{x}, \bm{y}$ are best responses.
\end{lemma}

\begin{proof}
    Consider, for $0 \le t \le 1$:
        \begin{align*}
        & f(t) = \uparp{c}{\bm{z}} = \uparp{c}{t \cdot \bm{x} + (1 - t) \cdot \bm{y}}
        & \\
        & = \frac{\bm{Q^c} \cdot (\bm{w^{-c}} + t \cdot \bm{x} + (1 - t) \cdot \bm{y})}{\bm{Q^*} \cdot (\bm{w^{-c}} + t \cdot \bm{x} + (1 - t) \cdot \bm{y})}
        & \\
        & = \frac{a + t \cdot b + (1 - t) \cdot d}{A + t \cdot B + (1 - t) \cdot D}
    \end{align*}
    For $a = \bm{Q^c} \cdot \bm{w^{-c}}, b = \bm{Q^c} \cdot \bm{x}, d = \bm{Q^c} \cdot \bm{y}$ and $A = \bm{Q^*} \cdot \bm{w^{-c}}, B = \bm{Q^*} \cdot \bm{x}, D = \bm{Q^*} \cdot \bm{y}$.
    Now, it can be verified that
    \begin{align*}
        f'(t) = -\frac{(B+A) \cdot d - (D + A) \cdot b + (B - D) \cdot a}{((D - B) \cdot t - D - A)^2}
    \end{align*}
    Hence, the sign of $f'(t)$ is constant, and $f$ is strongly monotonic, or constant.

    If $\bm{x}, \bm{y}$ are best responses, they must result in identical utility, hence $f(0) = f(1)$, and the function is constant, hence $f(r) = f(0) = f(1)$ and $\bm{z}$ is also a best response.

    For the other direction, assume $\bm{z}$ is a best response, and at least one of $\bm{x}, \bm{y}$ is not, assuming without a loss of generality that $x$ is not. Then $f(r) \ge f(0), f(r) > f(1)$. However, this contradicts monotonicity, so $\bm{x}, \bm{y}$ both must be best responses.
\end{proof}

\begin{lemma}
    Let $\bm{z}$ be a feasible investment with a strictly positive investment in a set $J \subseteq I$ of issues, and let $\bm{x}$ be an investment with positive investments only in issues in $J$. 
    
    There exists $\epsilon > 0$ such that $\bm{y} = \bm{z} + \epsilon \cdot (\bm{x} - \bm{z})$ is a feasible investment.
\end{lemma}

\begin{proof}
    First, we find $\epsilon > 0$ for which the investment in every issue is not negative. 
    Since $z_i = 0$ means $x_i = 0$, for every $i$ such that $z_i = 0$ it holds that $z_i + \epsilon \cdot (x_i - z_i) \ge 0$. 
    Now, for every $z_j > 0$, it is straightforward from the Archimedean property that there exists $\delta_j > 0$ such that for every $\delta'_j \le \delta_j$, it holds that $z_j < \delta'_j \cdot (z_i - x_i) \ge 0$, hence $z_i + \epsilon \cdot (x_i - z_i) \ge 0$. We then take $\epsilon = \underset{j : z_j > 0}{\text{min }} \delta_j$.

    Second, we ensure that the total sum of the investment does not exceed the budget:

    \begin{align*}
        & \sum_{i \in I} y_i = \sum_{i \in I} (z + \epsilon \cdot (x - z))_i 
        & \\
        & = \sum_{i \in I} z_i + \epsilon \cdot (\sum_{i \in I} z_i - \sum_{i \in I} x_i) 
        & \\
        & = W^c + \epsilon \cdot (W^c - W^c) = W^c
    \end{align*}

    We conclude that $y$ is a feasible investment.
\end{proof}

We return to the proof of \Cref{frac:focus_optimal_iff_split_is}:

\begin{proof}
    Let $\bm{z}$ be a best response to $\bm{w^{-c}}$ with a strictly positive investment in a set $J \subseteq I$ of issues, and let $\bm{x}$ be a response with positive investments only in issues in $J$.

    By the above lemma, there exists $\epsilon > 0$ such that $\bm{y} = \bm{z} + \epsilon \cdot (\bm{x} - \bm{z})$ is a feasible investment.

    Since $\bm{z}$ is between $\bm{x}, \bm{y}$, by \Cref{frac:best_middle_response} it holds that $\bm{x}, \bm{y}$ are also best responses, and in particular $\bm{x}$ is.
    
    For the other direction, the proof is by induction. We assume that every response involves positive investment only in up to $n$ issues in $J$ is optimal, and show that every response with positive investment in up to $n+1$ issues in $J$ is optimal.

    Let $\bm{z}$ be an investment in $n+1$ issues in $J$, assumed without a loss of generality to be the first $n+1$ issues. Let $\bm{x} = (z_1 + z_{n+1}, z_2, z_3, ..., z_n, 0, 0, ..., 0)$ and $\bm{y} = (0, z_2, z_3, ..., z_n, z_1 + z_{n+1}, 0, 0, ..., 0)$. It can be seen that $\bm{z}$ is between $\bm{x}, \bm{y}$, and that $\bm{x}, \bm{y}$ each involves positive investments only in a set of $n$ issue, and must then be best responses. Hence, by \Cref{frac:best_middle_response} it holds that $\bm{z}$ is also a best response.

    The claim for $n=1$ holds by assumption.
\end{proof}

==> proofs/frac/optimal_focus_exists.tex <==
We prove the following lemmas before the main proof.

\begin{definition}
    We say that a function is \emph{derivative sign indifferent} in a convex domain $D \subseteq R^n$ if it is differentiable in D, and whether or not $\frac{\partial f(\bm{x})}{\partial \bm{x}_i} = 0$ is independent of $\bm{x}_i$.
\end{definition}

\begin{lemma}
    \label{frac:constant-function}
    Given a derivative sign indifferent function $f$ in $D \subseteq R^n$, such that $f$ has an extreme point $\bm{a}$ in the interior of $D$, then every $\bm{x} \in D$ is an extreme point, hence $f$ is constant.
\end{lemma}

\begin{proof}
    We know $\frac{\partial f(\bm{a})}{\partial \bm{a}_i} = 0, \forall 1 \le i \le n$.
    Let there be an arbitrary $\bm{d} \in D$ in the interior of $D$.
    We define $d^i_k = \begin{cases}
        d_k & k \le i \\
        a_k & \text{otherwise}
    \end{cases}$

    We can see that $\bm{d^0} = \bm{a}, \bm{d^n} = \bm{d}$. Then $\bm{d^0}$ is an extreme point. If $\bm{d^i}$ is an extreme point, then all the partial derivatives are zero, and be assumption when moving along the $i+1$ axis the partial derivative along this axis is zero, hence $\bm{d^{i+1}}$ is also an extreme point. We get by induction that $\bm{d^n} = \bm{d}$ is an extreme point, hence every point in the interior in an extreme point. Since the function is differentiable and specifically continuous, then every point is an extreme point. 
\end{proof}

\begin{definition}
    We say that a function with a convex domain $f: D \rightarrow R$ is \emph{semi curved} if for every $a, b \in D$, either $\forall 0 \le r \le 1, f(r \cdot a + (1-r) \cdot b) \le r \cdot f(a) + (1-r) \cdot f(b)$ or $\forall 0 \le r \le 1, f(r \cdot a + (1-r) \cdot b) \ge r \cdot f(a) + (1-r) \cdot f(b)$.
\end{definition}

That is, a function is semi curved if for every two points, all the points between them are above the line between them, or all the points are below these line.

\begin{theorem}
    a
\end{theorem}

\begin{definition}
    The \emph{concise investment representation} of a candidate $c$ in a set $J \subseteq I$ of issues with a \emph{default issue} $j \in J$ is denoted by $(x^{c, j, J}_i)_{j \ne i \in J}$. $\bm{x^{c, j, J}}$ represents the investment $\bm{w^c}(\bm{x^{c, j, J}})$, such that:

    \begin{align*}
        & w^c(\bm{x^{c, j, J}})_i = \begin{cases}
            x^{c, j, J}_i & j \ne i \in J \\
            W^c - \sum_{k \ne j} \bm{x}_k & i = j \\
            0 & i \not\in J
        \end{cases}
    \end{align*}

    In order for $\bm{w^c}(\bm{x^{c, j, J}})$ to be a feasible investment, we require that $x^{c, j, J}_{j'} \in D_{c, j, J} = \{x : x_{j'} \ge 0 \forall j \ne j' \in J, \sum_{j': j \ne j' \in J} x_{j'} \le W^c\}$
\end{definition}

It can be seen that $w^c(\bm{x})$ is a feasible investment, and all feasible investments can be represented this way.

\begin{lemma}
    \label{frac:utility_is_derivative_sign_indifferent}
    Given the investments of all candidates except $c$, $\bm{w^{-c}}$, and given a set $J$ of issues and an arbitrary $j \in J$, $f(\bm{x^{c, j, J}}) = \uparp{c}{\bm{w^{-c}} + w^c(\bm{x^{c, j, J}})}$ is derivative sign indifferent in $D_{c, j, J}$.
\end{lemma}


\begin{proof}
The utility of $c$ for an investment $\bm{w^c}$ of $c$ is:

\begin{align*}
    & \uparp{c}{\bm{w^c}} = \frac{\bm{Q^c} \cdot (\bm{w^{-c}} + \bm{w^c})}{\bm{Q^*} \cdot (\bm{w^{-c}} + \bm{w^c})} = \frac{B^c + \bm{Q^c} \cdot \bm{w^c}}{B^* + \bm{Q^*} \cdot \bm{w^c}}
\end{align*}

For $B^c = \bm{Q^c} \cdot \bm{w^{-c}}, B^* = \bm{Q^*} \cdot \bm{w^{-c}}$. 

Now, for every $i \in I$:

\begin{align*}
    & Q^c_i (B^* + \bm{Q^*} \cdot \bm{w^c}) - Q^*_i (B^c + \bm{Q^c} \cdot \bm{w^c})
    & \\
    & = Q^c_i (B^* + \sum_{k \in I} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \in I} Q^c_k \cdot w^c_k)
    & \\
    & = Q^c_i (B^* + Q^*_i \cdot w^c_i + \sum_{k \neq i} Q^*_k \cdot w^c_k)
    & \\
    & - Q^*_i (B^c + Q^c_i \cdot w^c_i + \sum_{k \neq i} Q^c_k \cdot w^c_k)
    & \\
    & = Q^c_i \cdot Q^*_i \cdot w^c_i + Q^c_i (B^* + \sum_{k \neq i} Q^*_k \cdot w^c_k)
    & \\
    & - Q^c_i \cdot w^c_i \cdot Q^*_i + Q^*_i (B^c + \sum_{k \neq i} Q^c_k \cdot w^c_k)
    & \\
    & = Q^c_i (B^* + \sum_{k \neq i} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \neq i} Q^c_k \cdot w^c_k)
\end{align*}

Hence

\begin{align*}
    & \frac{\partial \upar}{\partial w^c_i} = \frac{Q^c_i (B^* + \bm{Q^*} \cdot \bm{w^c}) - Q^*_i (B^c + \bm{Q^c} \cdot \bm{w^c})}{(B^* + \bm{Q^*} \cdot \bm{w^c})^2}
    & \\
    & = \frac{Q^c_i (B^* + \sum_{k \neq i} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \neq i} Q^c_k \cdot w^c_k)}{(B^* + \bm{Q^*} \cdot \bm{w^c})^2}
\end{align*}

Let $\bm{x} = \bm{x^{c, j, J}}$ for an arbitrary $j \in J$.

For every $j \neq i \in I$ it holds that:

\begin{align*}
    & \frac{\partial \upar^c}{\partial x_i} = \sum_{k \in J} \frac{\partial \upar^c}{\partial w^c_k} \cdot \frac{w^c_k}{\partial x_i}
    & \\
    & = \frac{\partial \upar^c}{\partial w^c_i} \cdot \frac{w^c_i}{\partial x_i}
    + \frac{\partial \upar^c}{\partial w^c_j} \cdot \frac{w^c_j}{\partial x_i}
    & \\
    & = \frac{\partial \upar^c}{\partial w^c_i}
    - \frac{\partial \upar^c}{\partial w^c_j}
\end{align*}

The denominator of both $\frac{\partial \upar^c}{\partial w^c_i}, \frac{\partial \upar^c}{\partial w^c_j}$ is $(B^* + \bm{Q^*} \cdot \bm{w^c})^2$. Let's subtract the nominators:

\begin{align*}
    & Q^c_i (B^* + \sum_{k \neq i} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \neq i} Q^c_k \cdot w^c_k)
    & \\
    & - Q^c_j (B^* + \sum_{k \neq j} Q^*_k \cdot w^c_k) + Q^*_j (B^c + \sum_{k \neq j} Q^c_k \cdot w^c_k)
    & \\
    & =
    Q^c_i (B^* + Q^*_j \cdot w^c_j + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k)
    & \\
    & - Q^*_i (B^c + Q^c_j \cdot w^c_j + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & - Q^c_j (B^* + Q^*_i \cdot w^c_i + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k)
    & \\
    & + Q^*_j (B^c + Q^c_i \cdot w^c_i + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & =
    Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & - Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) + Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & + Q^c_i \cdot Q^*_j \cdot w^c_j -Q^*_i \cdot Q^c_j \cdot w^c_j
    & \\
    & - Q^c_j \cdot Q^*_i \cdot w^c_i + Q^*_j \cdot Q^c_i \cdot w^c_i
    & \\
    & =
    Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & - Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) + Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & + Q^c_i \cdot Q^*_j \cdot w^c_j -Q^*_i \cdot Q^c_j \cdot w^c_j
    & \\
    & - Q^c_j \cdot Q^*_i \cdot w^c_i + Q^*_j \cdot Q^c_i \cdot w^c_i
\end{align*}

Now, the last two lines are equal to:

\begin{align*}
    & Q^c_i \cdot Q^*_j \cdot w^c_j -Q^*_i \cdot Q^c_j \cdot w^c_j
    & \\
    & - Q^c_j \cdot Q^*_i \cdot w^c_i + Q^*_j \cdot Q^c_i \cdot w^c_i
    & \\
    & =
    Q^c_i \cdot Q^*_j \cdot (W^c - \sum_{k \ne j} \bm{x}_k) -Q^*_i \cdot Q^c_j \cdot (W^c - \sum_{k \ne j} \bm{x}_k)
    & \\
    & - Q^c_j \cdot Q^*_i \cdot w^c_i + Q^*_j \cdot Q^c_i \cdot w^c_i
    & \\
    & =
    Q^c_i \cdot Q^*_j \cdot (W^c - x_i - \sum_{k \not\in \{i, j\}} \bm{x}_k) 
    & \\
    & - Q^*_i \cdot Q^c_j \cdot (W^c - x_i - \sum_{k \not\in \{i, j\}} \bm{x}_k)
    & \\
    & - Q^c_j \cdot Q^*_i \cdot x_i + Q^*_j \cdot Q^c_i \cdot x_i
    & \\
    & =
    Q^c_i \cdot Q^*_j \cdot (W^c - \sum_{k \not\in \{i, j\}} \bm{x}_k) 
    & \\
    & - Q^*_i \cdot Q^c_j \cdot (W^c - \sum_{k \not\in \{i, j\}} \bm{x}_k)
    & \\
    & - Q^c_i \cdot Q^*_j \cdot x_i + Q^*_i \cdot Q^c_j \cdot x_i
    & \\
    & - Q^c_j \cdot Q^*_i \cdot x_i + Q^*_j \cdot Q^c_i \cdot x_i
    & \\
    & = 
    Q^c_i \cdot Q^*_j \cdot (W^c - \sum_{k \not\in \{i, j\}} \bm{x}_k) 
    & \\
    & - Q^*_i \cdot Q^c_j \cdot (W^c - \sum_{k \not\in \{i, j\}} \bm{x}_k)
\end{align*}

Finally the nominator of $\frac{\partial \upar^c}{\partial x_i} = \frac{\partial \upar^c}{\partial w^c_i} - \frac{\partial \upar^c}{\partial w^c_j}$ is, with $(B^* + \bm{Q^*} \cdot \bm{w^c})^2$ as the denominator:

\begin{align*}
    & Q^c_i (B^* + \sum_{k \neq i} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \neq i} Q^c_k \cdot w^c_k)
    & \\
    & - Q^c_j (B^* + \sum_{k \neq j} Q^*_k \cdot w^c_k) + Q^*_j (B^c + \sum_{k \neq j} Q^c_k \cdot w^c_k)
    & \\
    & =
    Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & - Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) + Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & + Q^c_i \cdot Q^*_j \cdot w^c_j -Q^*_i \cdot Q^c_j \cdot w^c_j
    & \\
    & - Q^c_j \cdot Q^*_i \cdot w^c_i + Q^*_j \cdot Q^c_i \cdot w^c_i
    & \\
    & =
    Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) - Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & - Q^c_i (B^* + \sum_{k \not\in \{i, j\}} Q^*_k \cdot w^c_k) + Q^*_i (B^c + \sum_{k \not\in \{i, j\}} Q^c_k \cdot w^c_k)
    & \\
    & + Q^c_i \cdot Q^*_j \cdot (W^c - \sum_{k \not\in \{i, j\}} \bm{x}_k) 
    & \\
    & - Q^*_i \cdot Q^c_j \cdot (W^c - \sum_{k \not\in \{i, j\}} \bm{x}_k)
\end{align*}

Hence, the nominator of $\frac{\partial \upar^c}{\partial x_i}$ is independent of $x_i$, and the denominator $(B^* + \bm{Q^*} \cdot \bm{w^c})^2$ is always positive, hence $f$ is derivative sign indifferent in $D_{c, j, J}$.

\end{proof}

The following is the proof for \Cref{frac:optimal_focus_exists}.

\begin{proof}
Let $\bm{x}$ be a vector such that $\bm{w^c}(\bm{x})$ is an optimal response that involves a positive investment in a set of issues $J$, and $j$ be an arbitrary issue in $J$. $x$ is an extreme point in the interior of $D_{c, j, J}$, with respect to the utility function of $c$. Then, by \Cref{frac:utility_is_derivative_sign_indifferent}, the conditions of $\Cref{frac:constant-function}$ hold and the function is constant, hence every investment only in issues from $J$ is an optimal investment.

\end{proof}

==> proofs/max/2_candidates_frac_equilbirium.tex <==
\begin{proof}
    The proof is done by a similar manner to that of \Cref{plus:2_candidates_frac_equilbirium}.
\end{proof}

==> proofs/max/best_response_doesnt_exist.tex <==
\begin{proof}

Consider the following game:

\begin{table}[h]
\centering
%\footnotesize
\begin{tabular}{@{\extracolsep{4pt}}rrrr}
\toprule
& $Q^{c_1}_i$ & $Q^{c_2}_i$ & $Q^{c_3}_i$ \\ 
\midrule
$1$ & $10$ & $0$ & $11$ \\
$2$ & $10$ & $9$ & $9$ \\
$3$ & $0$ & $0$ & $100$ \\
$W^c$ & $1$ & $0$ & $1$ \\
\bottomrule
\end{tabular}\\[3mm]
\end{table}



    
\end{proof}

==> proofs/model/legal_probabilities.tex <==
\begin{proof}
We know that

\begin{align*}
    & p^v(c, \bm{w}) = \sum_{i\in I} q^v_i(c) \cdot s_i^v(\bm{w})
    & \\
    & = \sum_{i\in I} q^v_i(c) \cdot \frac{s_i^v(w_i)}{\sum_{j\in I}s_j^v(w_j)} 
    & \\
    & = \sum_{i\in I} q^v_i(c) \cdot \frac{\rho_i w_i+s_i^v(0)}{\sum_{j\in I}(\rho_j w_j+s_j^v(0))}
\end{align*}

Since all the terms in the equation are non-negative, the result is non-negative as well. In addition:

\begin{align*}
    & \sum_{c \in C} p^v(c,\bm{w}) = \sum_{c \in C} \sum_{i\in I} q^v_i(c) \cdot s_i^v(\bm{w}) 
    & \\
    & = \sum_{i\in I} s_i^v(\bm{w}) \sum_{c \in C} q^v_i(c) \le \sum_{i\in I} s_i^v(\bm{w}) = 1
\end{align*}

When $\sum_{c\in C}q_i^v(c)=1$ the inequality becomes strict.

\end{proof}

==> proofs/pres/splitted_best.tex <==
\begin{proof}

Consider the following game:

\begin{table}[h]
\centering
%\footnotesize
\begin{tabular}{@{\extracolsep{4pt}}rrrr}
\toprule
& $c_1$ & $c_2$ & $c_3$ \\ 
\midrule
$Q^c_1$ & $1$ & $2$ & $0$ \\
$Q^c_2$ & $1$ & $0$ & $2$ \\
$W^c$ & $1$ & $0$ & $0$ \\
\bottomrule
\end{tabular}\\[3mm]
\end{table}

The only way for $c_1$ to win (partially) is to invest half in $1$ and half in $2$, which is the only best response.

\end{proof}
